SSAP: A Shape-Sensitive Adversarial Patch for Comprehensive Disruption of Monocular Depth Estimation in Autonomous Navigation Applications

Monocular depth estimation (MDE) has advanced significantly, primarily through the integration of convolutional neural networks (CNNs) and more recently, Transformers. However, concerns about their susceptibility to adversarial attacks have emerged, especially in safety-critical domains like autonomous driving and robotic navigation. Existing approaches for assessing CNN-based depth prediction methods have fallen short in inducing comprehensive disruptions to the vision system, often limited to specific local areas. In this paper, we introduce SSAP (Shape-Sensitive Adversarial Patch), a novel approach designed to comprehensively disrupt monocular depth estimation (MDE) in autonomous navigation applications. Our patch is crafted to selectively undermine MDE in two distinct ways: by distorting estimated distances or by creating the illusion of an object disappearing from the system's perspective. Notably, our patch is shape-sensitive, meaning it considers the specific shape and scale of the target object, thereby extending its influence beyond immediate proximity. Furthermore, our patch is trained to effectively address different scales and distances from the camera. Experimental results demonstrate that our approach induces a mean depth estimation error surpassing 0.5, impacting up to 99% of the targeted region for CNN-based MDE models. Additionally, we investigate the vulnerability of Transformer-based MDE models to patch-based attacks, revealing that SSAP yields a significant error of 0.59 and exerts substantial influence over 99% of the target region on these models.

==> draft.tex <==
The study conducted by the authors involved a comprehensive empirical investigation into the impact of catastrophic forgetting on the hidden representations of neural networks. They employed representational similarity measures \cite{kornblith2019similarity, raghu2017svcca} and conducted layer freezing and layer reset experiments. The results of their investigation indicated that deeper layers within the neural network were the main contributors to the phenomenon of forgetting. These deeper layers underwent the most significant changes during sequential training, leading to the observed effects of catastrophic forgetting.




==> setup.tex <==
%=====================
\section{Experimental Setup}
%=====================
\label{sec:setup}

In order to assess the effectiveness of our proposed attack, we analyzed vulnerabilities of two DNN models;  The self-supervised depth prediction models chosen based on their practicality and open source codes.

\textbf{Networks:}
DiverseDepth \cite{Wei2021CVPR} trained on depth prediction on multiple data sources including high-quality LiDAR sensor data \cite{Zamir_2018_CVPR}, and low-quality web stereo data \cite{Katrin2019,Chaoyang2019, xian2020structure}. 
%As these datasets have varied depth ranges and web stereo datasets contain unknown depth scale and shift, we propose an image-level normalized regression (ILNR) loss to address this issue. Moreover, we propose a pair-wise normal regression (PWN) loss to improve local geometric features.

The model has a backbone ResNet-50 and ResNet-101. 

Monodepth2 \cite{monodepth2} is based on the general U-Net architecture, i.e. an encoder-decoder network, enabling the representation of both deep abstract features as well as local information. The ResNet18 \cite{resnet} pretrained on ImageNet \cite{imagenet} was used as the encoder and the decoder was based on several convolution and upsampling layers with skip connections used to decode the output back to the input resolution.

\textbf{Datasets:} The patch was trained on indoor scenes from NYUv2 dataset \cite{nyuv2}. NYUv2 includes 654 images of different Indoor scenes (e.g., Bedroom, office)

The target depth maps were designed as if target objects were removed from the scenes.

==> suplementary.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{figures/results_pedestriant.pdf}
\caption{Impact of SSAP on pedestrian/cyclist class for CNN-based MDE. The cyclist seamlessly blends with the background.}
\label{results_ped}
\end{figure}
